BugSwarm: Mining and Continuously Growing a Dataset of Reproducible Failures and Fixes

Fault-detection, localization, and repair methods are vital to software quality; but it is difficult to evaluate their generality, applicability, and current effectiveness. Large, diverse, realistic datasets of durably-reproducible faults and fixes are vital to good experimental evaluation of approaches to software quality, but they are difficult and expensive to assemble and keep current. Modern continuous-integration (CI) approaches, like Travis-CI, which are widely used, fully configurable, and executed within custom-built containers, promise a path toward much larger defect datasets. If we can identify and archive failing and subsequent passing runs, the containers will provide a substantial assurance of durable future reproducibility of build and test. Several obstacles, however, must be overcome to make this a practical reality. We describe BugSwarm, a toolset that navigates these obstacles to enable the creation of a scalable, diverse, realistic, continuously growing set of durably reproducible failing and passing versions of real-world, open-source systems. The BugSwarm toolkit has already gathered 3,091 fail-pass pairs, in Java and Python, all packaged within fully reproducible containers. Furthermore, the toolkit can be run periodically to detect fail-pass activities, thus growing the dataset continually.

==> classification_figures.tex <==
% !TEX root = main.tex

\definecolor{python}{HTML}{FF7670}
\definecolor{java}{HTML}{7E8095}
\section{Classification}
\label{sec:classification}
This is the classification section
\pgfplotsset{width=7cm,compat=newest}
\begin{figure}\label{fig:lang_error}
        \caption{Top 10 Frequent Errors}
        \begin{tikzpicture}
        \begin{axis}[xbar,
        xbar=-\textwidth/128,
        axis x line*=bottom,
        axis y line*=left,
        xmin=-7,xmax=200,
        height=5cm, 
        width=\textwidth/3,
        bar width=\textwidth/120,
        xlabel={Number of Occurrences},
        legend style={at={(0.9,0.3)}, anchor=north,legend columns=-1},
        symbolic y coords = {SyntaxError,IOException,ImportError,TypeError,RuntimeException,ValueError,AttributeError,NullPointerException,AssertionError,jAssertionError},
        ytick = {jAssertionError,AssertionError,NullPointerException,AttributeError,%
        ValueError,RuntimeException,TypeError,ImportError,IOException,SyntaxError},
        yticklabels = {AssertionError,AssertionError,NullPointerException,AttributeError,%
        ValueError,RuntimeException,TypeError,ImportError,IOException,SyntaxError},
        y tick label style={font=\small, rotate=0, align=right, anchor=east},
        nodes near coords,
        nodes near coords align={horizontal}          
        ]
	
\addplot[java,fill] coordinates {(182,jAssertionError)};
\addplot[python,fill] coordinates {(158,AssertionError)};
\addplot[java,fill] coordinates {(70,NullPointerException)};
\addplot[python,fill] coordinates {(67,AttributeError)};
\addplot[python,fill] coordinates {(56,ValueError)};
\addplot[java,fill] coordinates {(48,RuntimeException)};
\addplot[python,fill] coordinates {(43,TypeError)};
\addplot[python,fill] coordinates {(42,ImportError)};
\addplot[java,fill] coordinates {(36,IOException)};
\addplot[python,fill] coordinates {(35,SyntaxError)};
\legend{$java$,$python$}
\end{axis}
\end{tikzpicture}   
\end{figure}

\begin{figure}\label{fig:py_error_10}
	\caption{Most Frequent Python Errors}
        \begin{tikzpicture}
        \begin{axis}[xbar,
        xbar=-\textwidth/128,
        axis x line*=bottom,
        axis y line*=left,
        xmin=-7,xmax=200,
        height=5cm, 
        width=\textwidth/3,
        bar width=\textwidth/120,
        xlabel={Number of Occurrences},
        symbolic y coords = {FileNotFoundError,NullPointerException,IndentationError,NameError,%
        SyntaxError,ImportError,TypeError,ValueError,AttributeError,AssertionError},
        ytick={FileNotFoundError,NullPointerException,IndentationError,NameError,SyntaxError,ImportError,TypeError,ValueError,AttributeError,AssertionError},
        yticklabels = {FileNotFoundError,NullPointerException,IndentationError,NameError,SyntaxError,ImportError,TypeError,ValueError,AttributeError,AssertionError},
        y tick label style={font=\small, rotate=0, align=right, anchor=east},
        nodes near coords,
        nodes near coords align={horizontal}          
        ]
\addplot coordinates {(17,FileNotFoundError)
(20,NullPointerException)
(21,IndentationError)
(30,NameError)
(35,SyntaxError)
(42,ImportError)
(43,TypeError)
(56,ValueError)
(67,AttributeError)
(158,AssertionError)};
\end{axis}
\end{tikzpicture}     

\end{figure}

\begin{figure}\label{fig:java_error_10}
		\caption{Most Frequent Java Exceptions}
        \begin{tikzpicture}
        \begin{axis}[xbar,
        xbar=-\textwidth/128,
        axis x line*=bottom,
        axis y line*=left,
        xmin=-7,xmax=200,
        height=5cm, 
        width=\textwidth/3,
        bar width=\textwidth/120,
        xlabel={Number of Occurrences},
        symbolic y coords = {EOFException,InvocationTargetException,SocketException,%
        NumberFormatException,IllegalArgumentException,IllegalStateException,%
        IOException,RuntimeException,NullPointerException,AssertionError},
        ytick={EOFException,InvocationTargetException,SocketException,%
        NumberFormatException,IllegalArgumentException,IllegalStateException,%
        IOException,RuntimeException,NullPointerException,AssertionError},
        yticklabels = {EOFException,InvocationTargetException,SocketException,%
        NumberFormatException,IllegalArgumentException,IllegalStateException,%
        IOException,RuntimeException,NullPointerException,AssertionError},
        y tick label style={font=\small, rotate=0, align=right, anchor=east},
        nodes near coords,
        nodes near coords align={horizontal}          
        ]
\addplot coordinates {(11,EOFException)(12,InvocationTargetException)(16,SocketException)(18,NumberFormatException)(23,IllegalArgumentException)(28,IllegalStateException)(36,IOException)(48,RuntimeException)(70,NullPointerException)(182,AssertionError)};
\end{axis}
\end{tikzpicture}   
\end{figure}

\begin{figure}\label{fig:diffsize_histogram}
        \caption{A Histogram of diff sizes}
        \begin{tikzpicture}
        \begin{axis}[
        ybar=-\textwidth/65,
        axis x line*=bottom,
        axis y line*=left,
        height=5cm, 
        ymin=-5,
        width=\textwidth/2,
        bar width=\textwidth/65,
        ylabel={Number of occurrences},
        xlabel={Number of changes made},
        symbolic x coords = {1-5,6-10,11-20,21-40,41-60,61-100,101-150,151-200,201-250,251-300},
        xtick = {1-5,6-10,11-20,21-40,41-60,61-100,101-150,151-200,201-250,251-300},
        x tick label style={font=\small, rotate=75, align=right, anchor=east},
  enlarge y limits=0.01,
        nodes near coords,
                nodes near coords align={vertical}          
        ]
    \addplot coordinates 
	{(1-5,436)
(6-10,246)
(11-20,255)
(21-40,177)
(41-60,110)
(61-100,101)
(101-150,73)
(151-200,22)
(201-250,21)
(251-300,26)}; 
\end{axis}
\end{tikzpicture}   
\end{figure}

\begin{figure}\label{fig:diffcount_histogram}
        \caption{A Histogram of diff count}
        \begin{tikzpicture}
        \begin{axis}[
        ybar=-\textwidth/65,
        axis x line*=bottom,
        axis y line*=left,
        height=5cm, 
        ymin=-5,
        width=\textwidth/2.5,
        bar width=\textwidth/65,
        ylabel={Number of occurrences},
        xlabel={Number of files changed},
        symbolic x coords = {1-5,6-10,11-25,26-50,51-100,101-150,151-200,201-3000},
        xtick = {1-5,6-10,11-25,26-50,51-100,101-150,151-200,201-3000},
        x tick label style={font=\small, rotate=75, align=right, anchor=east},
  enlarge y limits=0.01,
        nodes near coords,
                nodes near coords align={vertical}          
        ]
    \addplot coordinates 
	{(1-5,981)
(6-10,516)(11-25,194)
(26-50,85)
(51-100,36)
(101-150,18)
(151-200,15)
(201-3000,5)}; 
\end{axis}
\end{tikzpicture}   
\end{figure}

\begin{figure}\label{fig:failedtest_histogram}
        \caption{A Histogram of failed tests}
        \begin{tikzpicture}
        \begin{axis}[
        ybar=-\textwidth/65,
        axis x line*=bottom,
        axis y line*=left,
        height=5cm, 
        ymin=-5,
        width=\textwidth/2.5,
        bar width=\textwidth/65,
        ylabel={Number of occurrences},
        xlabel={Number of tests failed},
        symbolic x coords = {1,2-5,6-10,11-20,21-30,31-40,41-50},
        xtick = {1,2-5,6-10,11-20,21-30,31-40,41-50},
        x tick label style={font=\small, rotate=75, align=right, anchor=east},
  enlarge y limits=0.01,
        nodes near coords,
                nodes near coords align={vertical}          
        ]
    \addplot coordinates 
	{(1,371)
(2-5,193)
(6-10,44)
(11-20,14)
(21-30,6)
(31-40,13)
(41-50,13)}; 
\end{axis}
\end{tikzpicture}   
\end{figure}


\begin{figure}\label{fig:total_loc}
\caption{Project Size (in SLOC)}
\begin{tikzpicture} 
\begin{axis}[xlabel=Lines of Code, ylabel=Number of Projects] 
\addplot table [x=num_loc, y=num_projects,col sep=tab]{truncated_loc.dat}; 
\end{axis} 
\end{tikzpicture}
\end{figure}

\textbf{Statistics for Project Size:} 

Mean: 80327 sloc

Median: 59211 sloc

Min: 460 sloc

Max: 486603 sloc

\begin{table*}[t]
\small
\label{table:code_errors}
\caption{Confidence Values for Code Errors}
\begin{center}
\setlength{\tabcolsep}{4pt}
    \begin{tabular}{lrrrrr}
\toprule
    & \multicolumn{4}{c}{Confidence Score}\\
    \cmidrule{2-6}
 Language & 100\% & $>=$75\% & $>=$50\% & $>=$25\% & $<25$\%\\ 
 \midrule
Python & 303 tags (75.37 \%) & 30 tags (7.46 \%) & 37 tags (9.20 \%) & 32 tags (7.96 \%) & 0 tags (0.00 \%)\\ 
Java & 25 tags (2.29 \%) & 199 tags (18.19 \%) & 810 tags (74.04 \%) & 60 tags (5.48 \%) & 0 tags (0.00 \%)\\ 
\midrule
Total & 328 tags (21.93 \%) & 229 tags (15.31 \%) & 847 tags (56.62 \%) & 92 tags (6.15 \%) & 0 tags (0.00 \%)\\ 
    \bottomrule
\end{tabular}
\end{center}
\end{table*}

\begin{table*}[t]
\small
\label{table:test_errors}
\caption{Confidence Values for Test Errors}
\begin{center}
\setlength{\tabcolsep}{4pt}
    \begin{tabular}{lrrrrr}
\toprule
    & \multicolumn{4}{c}{Confidence Score}\\
    \cmidrule{2-6}
 Language & 100\% & $>=$75\% & $>=$50\% & $>=$25\% & $<25$\%\\ 
 \midrule
Python & 113 tags (36.93 \%) & 8 tags (2.61 \%) & 92 tags (30.07 \%) & 53 tags (17.32 \%) & 40 tags (13.07 \%)\\ 
Java & 187 tags (36.10 \%) & 55 tags (10.62 \%) & 163 tags (31.47 \%) & 80 tags (15.44 \%) & 33 tags (6.37 \%)\\ 
\midrule
Total & 300 tags (36.41 \%) & 63 tags (7.65 \%) & 255 tags (30.95 \%) & 133 tags (16.14 \%) & 73 tags (8.86 \%)\\ 
    \bottomrule
\end{tabular}
\end{center}
\end{table*}

\begin{table*}[t]
\small
\label{table:build_errors}
\caption{Confidence Values for Build Errors}
\begin{center}
\setlength{\tabcolsep}{4pt}
    \begin{tabular}{lrrrrr}
\toprule
    & \multicolumn{4}{c}{Confidence Score}\\
    \cmidrule{2-6}
 Language & 100\% & $>=$75\% & $>=$50\% & $>=$25\% & $<25$\%\\ 
 \midrule
Python & 2 tags (20.00 \%) & 0 tags (0.00 \%) & 6 tags (60.00 \%) & 0 tags (0.00 \%) & 2 tags (20.00 \%)\\ 
Java & 70 tags (34.48 \%) & 3 tags (1.48 \%) & 26 tags (12.81 \%) & 11 tags (5.42 \%) & 93 tags (45.81 \%)\\ 
\midrule
Total & 72 tags (33.80 \%) & 3 tags (1.41 \%) & 32 tags (15.02 \%) & 11 tags (5.16 \%) & 95 tags (44.60 \%)\\ 
    \bottomrule
\end{tabular}
\end{center}
\end{table*}
%%%%%%% THE PAIRS VS PROJECTS GRAPHS
\begin{figure}
\begin{tikzpicture} \label{fig:pairs_projects}
\begin{axis}[ybar stacked,
symbolic x coords = {1-10,11-20,21-50,51-100,101-200,201-500,501-5675},
xtick={1-10,11-20,21-50,51-100,101-200,201-500,501-5675}, 
xlabel={Number of Pairs},
ylabel= {Number of Projects},
x tick label style={font=\small, rotate=75, align=right, anchor=east},
nodes near coords,
legend style={at={(0.155,1)}, anchor=north,legend columns=1},] 
\addplot coordinates {(1-10,25)
(11-20,26)
(21-50,50)
(51-100,37)
(101-200,19)
(201-500,17)
(501-5675,8)};
\addplot coordinates {(1-10,10)
(11-20,6)
(21-50,19)
(51-100,27)
(101-200,34)
(201-500,23)
(501-5675,32)}; 
\legend{$java$,$python$}
\end{axis} 
\end{tikzpicture}
\end{figure}


%%%%%%%%%%%%%%PIE
\begin{figure}\label{fig:pie}
\caption{Pie chart about XYZ}
\begin{tikzpicture}
\pie[after  number =\% ,color={white,lightgray,gray,darkgray}, rotate=-60]{42/Unavailable, 22/To reproduce, 19/No Image, 17/Uses VM}
\end{tikzpicture}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%UNFILTERED/UNFILTERED-PR FIGURES%%%%%%%%%

%Cumulative # of pairs
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				xlabel = Number of pairs,
				x label style={at={(1, 0)}},
				ylabel = Number of projects,
				y label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				xmax=750,
				ymin=0,
%				ymax=75,
				ytick={25, 50, 75, 100, 125, 150, 175, 200},
				xtick={100, 200, 300, 400, 500, 600, 700, 800}
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[meta=label] {figures/data/cumulative_unfiltered.tsv};
		\addplot[red,mark=*] plot[error bars/.cd, y dir=minus,y fixed relative=1, x dir=minus,x fixed relative=1, error mark=none] coordinates { (160,33)};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Cumulative Unfiltered per Project}
	\label{fig:miner-cumulative}
\end{figure}

%Percentage of pairs
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				xlabel = Percentage of pairs,
				x label style={at={(1, 0)}},
				ylabel = Number of projects,
				y label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				xmax=100,
				ymin=0,
				ymax=300,
				ytick={50,100, 150, 200, 250, 300},
				xticklabel={\pgfmathprintnumber\tick\%},
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[x=x, y=y, meta=label] {figures/data/fail-pass-percent-per-language.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Percentage Unfiltered per Project}
	\label{fig:miner-percentage}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%FAIL-PASS%%%%%%%%%%%%%
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				ylabel = Percentage of fail-pass pairs,
				y label style={at={(1, 0)}},
				xlabel = Number of projects,
				x label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				ymax=100,
				ymin=0,
				xmax=300,
				yticklabel={$>=$\pgfmathprintnumber\tick\%},
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[x=num_pairs, y=percent, meta=label] {figures/data/fail-pass-percent-per-language-cumulative.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Percentage of Fail-Pass Pairs in Projects}
	\label{fig:fail-pass-percentage}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%REPRODUCED FIGURES%%%%%%%%%
%Cumulative # of pairs
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				xlabel = Number of pairs,
				x label style={at={(1, 0)}},
				ylabel = Number of projects,
				y label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				ymin=0,
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[x=num_pairs, y=num_projects, meta=label] {figures/data/reproduced-number-per-language-cumulative-sparse.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Number of Reproduced Pairs in Projects}
	\label{fig:reproduced-cumulative}
\end{figure}
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[
				legend cell align={left},
				ylabel = Number of pairs,
				y label style={at={(0, 1)}},
				xlabel = Number of projects,
				x label style={at={(1, 0)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				ymode=log,
		        log ticks with fixed point,
				xmax=100,
				ymin=-1,
				ymax=500,
ytick={0,1,5, 10, 50, 100, 500},
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[y=num_pairs, x=num_projects, meta=label] {figures/data/reproduced-number-per-language-cumulative-sparse.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Number of Reproduced Pairs in Projects}
	\label{fig:reproduced-cumulative-axis}
\end{figure}
%Percentage of pairs
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				xlabel = Percentage of reproducible pairs,
				x label style={at={(1, 0)}},
				ylabel = Number of projects,
				y label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				xmax=100,
				ymin=0,
				ymax=90,
				ytick={10, 20, 30, 40, 50, 60, 70, 80, 90},
				xticklabel={$>=$\pgfmathprintnumber\tick\%},
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[x=percent, y=num_pairs, meta=label] {figures/data/reproduced-percent-per-language-cumulative.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Percentage of Reproduced Pairs in Projects}
	\label{fig:reproduced-percentage}
\end{figure}
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
            \large
			\begin{axis}[axis lines=middle,
				legend cell align={left},
				ylabel = Percentage of reproducible pairs,
				y label style={at={(1, 0)}},
				xlabel = Number of projects,
				x label style={at={(0, 1)}},
                                ylabel near ticks,
                                xlabel near ticks,
				xmin=0,
				ymax=100,
				ymin=0,
				xmax=90,
				xtick={10, 20, 30, 40, 50, 60, 70, 80, 90},
				yticklabel={$>=$\pgfmathprintnumber\tick\%},
				]
		\legend{Java, Python}
		\addplot[
		scatter,
		only marks,
		point meta=explicit symbolic,
		scatter/classes={
		j={mark=*,red},%
		p={mark=*,blue}},
		]
			table[x=num_pairs, y=percent, meta=label] {figures/data/reproduced-percent-per-language-cumulative.tsv};
		\end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Percentage of Reproduced Pairs in Projects}
	\label{fig:reproduced-percentage-changed-axes}
\end{figure}


==> code_build_test.tex <==
We also classified artifacts as build or test errors. We analyzed the diffs for the artifact, and if changes were made in test files or build configuration files (eg. POM or travis files) then they were labelled as test and build errors respectively. However, a simple binary classification could result in a large number of false positives since commits often include multiple files that are not directly related to the fix. To counter this, we assigned each artifact a confidence score to measure the influence of a particular error on the status of the build; 
A 100\% confidence score would indicate that the artifact failed definitively due to the corresponding error. 

We observed that 19.44\% of all artifacts had a 100\% score for test errors, indicating that the artifact did not pass solely due to test errors. Similarly, 5\% of all artifacts failed due to errors in build configuration. 


==> figures.tex <==
% !TEX root =  main.tex

% \tikzset{mark options={mark size=1}}



\begin{comment}
\begin{figure}
	\begin{center}
		\begin{tikzpicture}[scale=0.6]
		  \large
		  \begin{axis}
		    [
		    boxplot/draw direction=y,
		    ylabel=Job pairs,
		    y label style={at={(1, 0)}},
		    ylabel near ticks,
		    ymode=log,
		    xtick={1, 2, 3, 4, 5},
		    xticklabels={F. Jobs, Mined, Avail., Image, Quay},
		    ]
		    \addplot+[
		    boxplot prepared={
		      median=494,
		      upper quartile=1568.75,
		      lower quartile=155.75,
		      upper whisker=49870,
		      lower whisker=1
		    }, color = black
		    ] coordinates {};
		    \addplot+[
		    boxplot prepared={
		      median=99.5,
		      upper quartile=304.5,
		      lower quartile=36,
		      upper whisker=11207,
		      lower whisker=1
		    }, color = black
		    ] coordinates {};
		    \addplot+[
		    boxplot prepared={
		      median=71,
		      upper quartile=189.25,
		      lower quartile=19,
		      upper whisker=2634,
		      lower whisker=1
		    }, color = black
		    ] coordinates {};
		    \addplot+[
		    boxplot prepared={
		      median=42,
		      upper quartile=123,
		      lower quartile=9,
		      upper whisker=1815,
		      lower whisker=1
		    }, color = black
		    ] coordinates {};
		    \addplot+[
		    boxplot prepared={
		      median=5,
		      upper quartile=43.25,
		      lower quartile=1,
		      upper whisker=1815,
		      lower whisker=1
		    }, color = black
		    ] coordinates {};
		  \end{axis}
		\end{tikzpicture}
	\end{center}
	\caption{Effect of Various Filters}
        \label{fig:filter-effect}
\end{figure}
\end{comment}







==> long-related.tex <==
% !TEX root = main.tex

\section{Related Work}
\label{sec:related}
Most closely related to our work are defect repositories that aim to
provide experimental benchmarks for researchers interested in defect
location and repair.  \etc Speaking as a whole these repositories do
not exploit the continuous integration and virtualization mechanisms
(and in many cases pre-date the widespread adoption of these
techniques) and so do not achieve the same \textit{scale, diversity,
  and currency} and are not as \textit{durably reproducible}.

The Siemens test suite ~\citep{DBLP:conf/icse/HutchinsFGO94}, (7 small C
programs, less than 1000 lines, and about 130 manually seeded bugs) was among
the earliest; despite its obvious limitations, it was quite widely used.

BugBench ~\citep{Lu05bugbench:benchmarks} is one of the earliest datasets of
real-world bugs for evaluating bug detection tools. BugBench is limited in scale
and diversity, consisting of 7 C/C++ memory and concurrency bugs found across 10
open-source projects. Each buggy program version includes tests that trigger the
corresponding bug. Unlike \bugswarm, BugBench is manually constructed.

iBugs ~\citep{DBLP:conf/kbse/DallmeierZ07} is a real-world dataset
drawn from the 5-year history of a single project, the AspectJ
compiler. It comprises 369 faulty versions of the project, including
223 that have at least one associated test. iBugs identifies bug fixes
by searching for keywords such as ``Fixed'' in commit messages. Then,
iBugs extracts the pre-fix and post-fix versions, builds each version,
and executes test suites, when available. Although limited in scale
and diversity, iBugs provides detailed metadata about the fix such as
the number of methods and classes changed as well as the specific
tokens affected by the change, including variable name changes. Such
data can be built from \bugswarm artifacts with some additional
effort.

The Software-artifact Infrastructure Repository (SIR)
~\citep{DBLP:journals/ese/DoER05} comprises source code, tests, and
defects from open-source projects along with needed infrastructure
(\eg automated build and test scripts). Currently, it consists of 85
projects in four languages, of which 64 (15 C, 1 C\#, 1 C++, and 47
Java) also include fault data; faults are real in 36 projects, seeded
in 23, and some combination of real, seeded, and mutated in the other
5. A project may contain multiple versions (min 1; median 1; mean
3.08; max 41), and each version may contain multiple faults. Projects
with fault data are mostly small: they range in size between 24 and
503,800 LOC (median 567.5; mean 16,940); and 1---1,999 files (median
8; mean 32).\footnote{Data aggregated from
  \href{http://sir.unl.edu/php/showfiles.php}{http://sir.unl.edu/php/showfiles.php}.} The total number of
defects reported in the paper is around 680, including both seeded and
real defects. SIR is over a decade old, very widely used, highly
influential, and has almost 900 citations to the original paper. It
provides a useful amount of scale, diversity, and archives sufficient
tooling for durable reproducibility. However, since it pre-dates CI
and \dockr, each defect datum therein is manually assembled. Thus, SIR
is difficult to scale up further and requires substantial effort to
keep current. Despite being much newer, \bugswarm already has many
more reproducible (\numJobPairArtifacts) defects; the automated mining
of CI and \dockr image artifacts lowers the cost of keeping the
current dataset growing and current.

Defects4J ~\citep{DBLP:conf/issta/2014} is a dataset of 357 real, reproducible
bugs from 5 large Java programs. Bugs are found from commit logs in version
history. Defects4J also provides manually constructed scripts for each project's
build and test; the whole setup relies on a functioning JVM. Defects4J provides
an interface for common tasks and provides support for a number of tools,
including code coverage tools. Despite being fairly recent, it has been very
influential, and is the most well-cited paper from ISSTA 2014.

By contrast, \bugswarm relies on virtualized, \dockr-packaged build and test
environments, automatically harvested from the cross-platform \tvis CI archives;
thus it is neither limited to Java, nor does it require manual assembly of build
and test tools. In addition to the test failing/passing pairs that Defects4J
provides, we also include build failures and even flaky tests. This allows
\bugswarm to achieve greater scale, (around \numJobPairArtifacts samples so far,
and growing) diversity and currency. We argue that the \dockr platform is likely
to be as durable as Java since \dockr has a great diversity of use-cases and
huge base of stakeholders; this durability would redound to \bugswarm as well.

Another recent paper by Urli \etal ~\cite{urli2018design} describes an approach
to mining builds that fail tests from \tvis. This work specializes in
Maven-based Java builds that are reproduced directly, without \dockr. They
reproduced an impressively large 3,552 Maven Java builds for the purpose of
automatic repair. Our \dockr-based approach allows other languages and build
systems, and our approach (with a dataset currently comprising a similarly large
set of durably reproducible builds, from \numJobPairArtifacts fail-pass pairs)
reflects our designed-in pursuit of a much higher level of diversity (See
~\cref{tab:diversity}). Like their approach, our approach is automated; it can
and is continually growing in scale while also providing increasing diversity.
Finally, the use of \dockr containers frees one from specific language, build
system, or runtime version constraints and arguably provides a more durable
level of reproducibility.

\textsc{ManyBugs} ~\citep{DBLP:journals/tse/GouesHSBDFW15} is a
benchmark for automated program repair that consists of 185
defects/fixes from nine large, popular OSS C projects. 
The defects are mined from the history of the top 20 C
projects found in open-source websites. Each defect/fix includes
tests, and is manually categorized. To facilitate the reproduction of
these defects, \textsc{ManyBugs} provides virtual machine
images. Unlike \bugswarm the process of mining and reproducing bugs
requires significant manual effort, and thus \textsc{ManyBugs} is not
as easy to extend. On the other hand, \textsc{ManyBugs} provides a
detailed bug categorization that can be useful for experiments, and
its artifacts are collected from C programs, a programming language
that \bugswarm could support with some extensions, since \tvis CI already
supports it. 

There are other, less related datasets of programs. The SPEC benchmarks
~\citep{spec-benchmarks} are designed to evaluate performance and energy
efficiency.
The DaCapo Java performance benchmarks ~\citep{DaCapo:paper} improve on the Java
SPEC benchmarks by carefully considering memory management systems and virtual
machines when evaluating performance. Sourcerer ~\cite{bajracharya2014sourcerer}
is a searchable dataset of open-source projects, with a focus on source code
structure; although it is a good jumping-off point for build and test, it is not
explicitly designed for durably reproducible build and test. Xu and Marinov
advocate the mining of large repositories of \dockr images to learn about
the characteristics of execution ecosystems ~\cite{xu2018mining}. \bugswarm
could be an enabler to achieve some of their goals.

We conclude this section by noting that the \bugswarm toolset supports the
creation of fully reproducible packages for any pair of commits for which the
\tvis builds are archived. There are tens of thousands of projects in \ghub that
use \tvis, so our toolkit enables the creation of datasets and enusing
experiments at a scale substantially larger than previous datasets allow.

\cbstart
Two recent papers also observe these challenges: Urli \etal
~\cite{urli2018design} focus on mining CI logs for defects, specifically for
Java, and point out the difficulty of processing CI logs and note the low rate
of reproducibility of observed fail-pass build pairs. Xu and Marinov
~\cite{xu2018mining} note the difficulties of mining and/or recreating \dockr
images.
\cbend

==> research-opportunities.tex <==

\section{Research Opportunities}
\todo[inline]{Remove claims that research opportunities are a contribution.}
One of the main contributions of \bugswarm along with the research
infrastructure and dataset is the large number of research
opportunities it opens. \bugswarm will provide a much larger and
realistic dataset for evaluating bug localization and automated
program repair techniques as well as conducting empirical studies of
failures, which include:

\mysec{Evaluating static \& dynamic analysis}
The goal is to evaluate the ability of static and dynamic methods to
warn of potential errors. By analyzing the relationship between
warnings with actual defect repairs \citep{rahman2014comparing}, one
can measure the specificity and accuracy of these analysis tools.

\mysec{Evaluating test generation methods}
Testing's goal is to find bugs; so the \bugswarm dataset would be very
useful to evaluate whether the tests generated by a given approach can
find bugs, and if so, what kinds of bugs, and under what conditions.

\mysec{Collecting defect-fix patterns} Another thrust of research has
been aimed at collecting defect-fixing patterns in datasets of defects
(e.g., \citep{kim2006memories,nguyen2010recurring}).  \bugswarm
provides a very large collection of defects \& repairs, further
boosting research in this area.

\mysec{Studying effects of CI practices} The PR model, and CI have
attracted quite a bit of interest of late (\citep{
  gousios2014exploratory,rigby2013convergent}). \bugswarm allows
evaluation of the relationship of process properties (ownership,
experience, \etc), on both static and dynamic properties of code, as
well as quality outcomes.

\mysec{Evaluating test selection and prioritization} When test sets
are large, and require a lot of human or computing resources to run,
it would be nice to select or prioritize those tests that are most
likely to expose bugs. This a very active area of research (e.g.,
\cite{graves2001empirical,rothermel1997safe}) that would benefit from
\bugswarm.

